Large Language Models to the Rescue: Reducing the Complexity in Scientific Workflow Development Using ChatGPT

Scientific workflow systems are increasingly popular for expressing and executing complex data analysis pipelines over large datasets, as they offer reproducibility, dependability, and scalability of analyses by automatic parallelization on large compute clusters. However, implementing workflows is difficult due to the involvement of many black-box tools and the deep infrastructure stack necessary for their execution. Simultaneously, user-supporting tools are rare, and the number of available examples is much lower than in classical programming languages. To address these challenges, we investigate the efficiency of Large Language Models (LLMs), specifically ChatGPT, to support users when dealing with scientific workflows. We performed three user studies in two scientific domains to evaluate ChatGPT for comprehending, adapting, and extending workflows. Our results indicate that LLMs efficiently interpret workflows but achieve lower performance for exchanging components or purposeful workflow extensions. We characterize their limitations in these challenging scenarios and suggest future research directions.

==> images/sw_example.tex <==
% \begin{figure}[t]
% \includegraphics[width=\textwidth]{images/sw_example_ninon.png}
% \centering
% \caption{Example bioinformatics workflow for differential gene expression analysis created by one domain expert recruited in our study. The figure highlights the conceptional schema of the workflow (left), it's implementation in nextflow (middle) as well as the implementation of one single step (right), i.e. reference genome alignment using the STAR tool. The workflow comprises seven computational steps in total. For each step the used tool is given in blue below the task description.}
% \label{fig:sw_example}
% \end{figure}


\begin{figure*}
    \centering
    \subfloat[][]{
        \includegraphics[height=0.5\textwidth]{images/sw_ninon_a.png}
        \label{fig:ninon_a}}
    \subfloat[][]{
        \includegraphics[height=0.5\textwidth]{images/sw_ninon_b.png}
        \label{fig:ninon_b}}
    \subfloat[][]{
        \includegraphics[height=0.5\textwidth]{images/sw_ninon_c.png}
        \label{fig:ninon_c}}
    \caption{Example bioinformatics workflow for differential gene expression analysis created by one domain expert recruited in our study. The figure highlights the conceptional schema of the workflow (a), its implementation in Nextflow (b), and the implementation of one single step (c), i.e., reference genome alignment using the STAR tool. The workflow comprises six computational steps in total. For each step the used tool is given in blue below the task description.}
    \label{fig:ninon}
\end{figure*}

==> table/tab_workflows.tex <==
\begin{table*}[htbp]
    \centering
    \caption{Overview about the used workflows for our first user study targeting the workflow comprehension capabilities of ChatGPT. We examine workflows from two different scientific domains, i.e. bioinformatics and earth observation, and two different workflow systems (Nextflow and Apache airflow). For each workflow we report the number of (high-level) steps and the number of used tools.}
        \begin{tabular}{clp{7.8cm}cc}
            \toprule
            \textbf{Domain}&\textbf{Workflow}&\textbf{Description}&\textbf{\#Steps}&\textbf{\#Tools}\\
                \hline

            \makecell[tl]{Bio-\\informatics}
    
                & \makecell[tl]{
                    WF1:\\crisprseq \cite{sanvicente2023crispr}\\
                    (\textit{Nextflow})
                }&
                \makecell*[t{{p{7.8cm}}}]{
                    A bioinformatics data pipeline for analyzing and evaluating gene editing experiments utilizing CRISPR-Cas9 mechanism for genome engineering. \\
                    Repository: \url{https://nf-co.re/crisprseq/2.0.0} (created 07/2022)
                }&
                6&
                9\\

            \cline{2-5}
            
            &
                \makecell[tl]{
                    WF2:\\RS-Star\\
                    (\textit{Nextflow})
                }&
                \makecell*[t{{p{7.8cm}}}]{
                    The general aim of this workflow is to perform differential gene expression analysis using RNA-seq data.\\
                    Repository: \url{https://github.com/Nine-s/nextflow_RS1_star} (created 11/2021)
                }&
                5&
                5\\

            \hline 

            \makecell[tl]{Earth\\observation}&
                \makecell[tl]{
                    WF3:\\FORCE2NXF-\\Rangeland \cite{lehmann2021force}\\
                    (\textit{Nextflow})
                }&
                \makecell*[t{{p{7.8cm}}}]{
                    This workflow focuses on analyzing long-term vegetation dynamics in the Mediterranean using the FORCE-toolkit. \\
                    Repository: \url{https://github.com/CRC-FONDA/FORCE2NXF-Rangeland} (created 11/2020)
                }&
                9&
                8\\

            \cline{2-5}

            &
                \makecell[tl]{
                    WF4:\\Grasslands\\
                    (\textit{Nextflow})
                }&
                \makecell*[t{{p{7.8cm}}}]{
                    This workflow provides information on long-term changes in ground cover fractions specific to grasslands in the Caucasus region. \\
                    Repository: \url{https://github.com/kelewinska/FONDA_trends-nf} (created 08/2023)
                }&
                6&
                3\\
                
            \cline{2-5}
            &
                \makecell[tl]{
                    WF5:\\Force\\
                    (\textit{Apache airflow})
                }&
                \makecell*[t{{p{7.8cm}}}]{
                    This workflow focuses on analyzing long-term vegetation dynamics in the Mediterranean using the FORCE-toolkit.\\
                    Repository: \url{https://github.com/CRC-FONDA/fonda-airflow-dags/tree/main} (created 02/2021)
                }&
                8&
                8\\
                \bottomrule
        \end{tabular}
    \label{tab:workflows}
\end{table*}
